Safety-Aware Cascade Controller Tuning Using Constrained Bayesian Optimization

This paper presents an automated, model-free, data-driven method for the safe tuning of PID cascade controller gains based on Bayesian optimization. The optimization objective is composed of data-driven performance metrics and modeled using Gaussian processes. We further introduce a data-driven constraint that captures the stability requirements from system data. Numerical evaluation shows that the proposed approach outperforms relay feedback autotuning and quickly converges to the global optimum, thanks to a tailored stopping criterion. We demonstrate the performance of the method in simulations and experiments. For experimental implementation, in addition to the introduced safety constraint, we integrate a method for automatic detection of the critical gains and extend the optimization objective with a penalty depending on the proximity of the current candidate points to the critical gains. The resulting automated tuning method optimizes system performance while ensuring stability and standardization

==> New version Safety-aware BO - arXiv/mystyle.tex <==
%===================== Packages ====================
%\usepackage[numbers]{natbib}
%\usepackage{natbib}
%\usepackage[noadjust]{cite}
% \usepackage[colorlinks=true]{hyperref}
\usepackage{amssymb, amsmath, amsfonts}
%\usepackage{  mathrsfs, color, bm}%, url,authblk,dsfont,
\usepackage{ graphicx, epstopdf}%, subfigure}%, subcaption}% , transparent,, pgfplots
\usepackage{algorithm,  multirow,titlecaps,algorithmicx} %, titlecaps,algorithmicx,
\usepackage[T1]{fontenc}
\usepackage{marvosym}
%\usepackage{verbatim}
%\usepackage{threeparttable}

\usepackage{tikzsymbols}
% Defining mathbbold font
\DeclareMathAlphabet{\mathbbold}{U}{bbold}{m}{n}

% For pseudocodes and algorithms
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage[noend]{algpseudocode} 
%=================================================
%\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
% \usepackage{algorithmic}
\usepackage{graphicx}
%\usepackage{textcomp}
\usepackage{xcolor}
%\usepackage{hyperref}
% for nice tables ...
%\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{courier}
\usepackage{float}
\usepackage{makecell}
\setcellgapes{5pt}
%\usepackage{subcaption}
%\captionsetup{compatibility=false}
%\usepackage[options ]{algorithm2e}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
%\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%		T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%==================== Commenting ==================
\newcommand{\cm}[1]{{\color{violet}{{[#1]}}}}
\newcommand{\cmb}[1]{{\color{blue}{#1}}}
\newcommand{\cmr}[1]{{\color{red}{#1}}}
\newcommand{\cmg}[1]{{\color{green}{#1}}}
\newcommand{\cmm}[1]{{\color{magenta}{#1}}}
\newcommand{\cmc}[1]{{\color{cyan}{#1}}}
\newcommand{\cmt}[1]{{\color{teal}{#1}}}
\newcommand{\cmp}[1]{{\color{purple}{#1}}}
%=================================================
\newcommand{\stiny}[1]{{\scalebox{.5}{#1}}}
\newcommand{\smtiny}[1]{{\scalebox{.63}{#1}}}
\newcommand{\sstiny}[1]{{\scalebox{.25}{#1}}}
%================= MATH Abbreviation ==============
%=============== Abbreviation ==================
\newcommand{\argmin}{{\mathrm{argmin}}}
\newcommand{\argmax}{{\mathrm{argmax}}}
\newcommand*{\argminOp}{\operatornamewithlimits{argmin}\limits}
\newcommand*{\argmaxOp}{\operatornamewithlimits{argmax}\limits}
\newcommand*{\minOp}{\operatornamewithlimits{min}\limits}
\newcommand*{\maxOp}{\operatornamewithlimits{max}\limits}

\newcommand{\tr}{{\mathsf{T}}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\iftrue%\iffalse %<-<-<-<-<-<-<-<-<-<-<-<-<-<-<
\newcommand{\zeromx}{{\mathbbold{0}}} %<<<<
\newcommand{\eye}{\mathbb{I}}
\else
\newcommand{\zeromx}{{\mathbf{0}}} %<<<<
\newcommand{\eye}{\mathbf{I}}
\fi%<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\vc}[1]{{ \mathrm{#1} }}
\newcommand{\mx}[1]{{ \mathrm{#1} }}
\newcommand*{\Times}{\operatornamewithlimits{\scalebox{1.5}{$\times$}}\limits}
\newcommand{\dom}{\mathrm{dom}}

%% __ mathscr of D, F, X, Y, Z,...
\newcommand{\Dscr}{{\mathscr{D}}}
\newcommand{\Fscr}{{\mathscr{F}}}
\newcommand{\Xscr}{{\mathscr{X}}}
\newcommand{\Yscr}{{\mathscr{Y}}}
\newcommand{\Zscr}{{\mathscr{Z}}}

%% __ mathcal of X, Y, Z,...
\newcommand{\Acal}{{\mathcal{A}}}
\newcommand{\Bcal}{{\mathcal{B}}}
\newcommand{\Ccal}{{\mathcal{C}}}
\newcommand{\Dcal}{{\mathcal{D}}}
\newcommand{\Ecal}{{\mathcal{E}}}
\newcommand{\Fcal}{{\mathcal{F}}}
\newcommand{\Gcal}{{\mathcal{G}}}
\newcommand{\Hcal}{{\mathcal{H}}}
\newcommand{\Ical}{{\mathcal{I}}}
\newcommand{\Jcal}{{\mathcal{J}}}
\newcommand{\Kcal}{{\mathcal{K}}}
\newcommand{\Lcal}{{\mathcal{L}}}
\newcommand{\Mcal}{{\mathcal{M}}}
\newcommand{\Ncal}{{\mathcal{N}}}
\newcommand{\Ocal}{{\mathcal{O}}}
\newcommand{\Pcal}{{\mathcal{P}}}
\newcommand{\Qcal}{{\mathcal{Q}}}
\newcommand{\Rcal}{{\mathcal{R}}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{{\mathcal{U}}}
\newcommand{\Wcal}{{\mathcal{W}}}
\newcommand{\Xcal}{{\mathcal{X}}}
\newcommand{\Ycal}{{\mathcal{Y}}}
\newcommand{\Zcal}{{\mathcal{Z}}}

%% __ mathbb of X, Y, Z,...
%\newcommand{\Bbb}{{\mathbb{B}}}
\newcommand{\Cbb}{{\mathbb{C}}}
\newcommand{\Dbb}{{\mathbb{D}}}
\newcommand{\Ebb}{{\mathbb{E}}}
\newcommand{\Fbb}{{\mathbb{F}}}
\newcommand{\Gbb}{{\mathbb{G}}}
\newcommand{\Hbb}{{\mathbb{H}}}
\newcommand{\Ibb}{{\mathbb{I}}}
\newcommand{\Jbb}{{\mathbb{J}}}
\newcommand{\Kbb}{{\mathbb{K}}}
\newcommand{\Lbb}{{\mathbb{L}}}
\newcommand{\Mbb}{{\mathbb{M}}}
\newcommand{\Nbb}{{\mathbb{N}}}
\newcommand{\Pbb}{{\mathbb{P}}}
\newcommand{\Qbb}{{\mathbb{Q}}}
\newcommand{\Rbb}{{\mathbb{R}}}
\newcommand{\Sbb}{{\mathbb{S}}}
\newcommand{\Tbb}{{\mathbb{T}}}
\newcommand{\Ubb}{{\mathbb{U}}}
\newcommand{\Vbb}{{\mathbb{V}}}
\newcommand{\Xbb}{{\mathbb{X}}}
\newcommand{\Ybb}{{\mathbb{Y}}}
\newcommand{\Zbb}{{\mathbb{Z}}}
\newcommand{\bbo}{\mathbbold{o}}
%\newcommand{\bbo}{\mathbb{o}}
\newcommand{\bbh}{\mathds{h}}
%\newcommand{\bbk}{\mathds{k}}
%\newcommand{\bbk}{\mathbbold{k}}
\newcommand{\bbk}{\mathbbm{k}}

%% __ hat of f, g
\newcommand{\hatf}{{\hat{f}}}
\newcommand{\hatg}{{\hat{g}}}
%_______________________________________________
\newcommand{\Max}{\max\limits}
\newcommand{\Min}{\min\limits}
\newcommand{\Sup}{\sup\limits}
\newcommand{\Inf}{\inf\limits}
\newcommand{\Sum}{\sum\limits}
\newcommand{\SumN}{\sum\limits_{i=1}^N}
\newcommand{\WWbar}{\widetilde{\mathbb{W}}}

%% __ other fonts (Probability)
\newcommand{\PP}{\mathds{P}}
\newcommand{\QQ}{\mathds{Q}}
\newcommand{\EE}{\mathds{E}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\KK}{\bm{\mathcal{K}}}
\newcommand{\GG}{\bm{\mathcal{G}}}
\newcommand{\II}{\mathcal{I}}
\newcommand{\JJ}{\mathcal{J}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\ZZ}{\mathcal{Z}}

%==================================================
%===================== Theorem ====================
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Propositon}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
%==================================================
%==================== Figures Path ================
%\graphicspath{{figures/}}
%==================================================
%===================== TODO List ==================
%\iftrue %<--
\iffalse
\let\labelindent\relax
\usepackage{enumitem}
\newlist{todolist}{itemize}{2}
\setlist[todolist]{label=$\square$}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\done}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}% 
	\hspace{-2.5pt}}
% for being done and remain in list!
\newcommand{\wontfix}{\rlap{$\square$}{\large\hspace{1pt}\xmark}} 
% for being conceled but remain in the list!
\fi 
%=================================================
%==== Modify style ===============================
\iftrue %<--
%\iffalse
	\usepackage{xcolor}
	\hypersetup{
		colorlinks,
		linkcolor={blue!55!black},
		citecolor={red!55!black},
		urlcolor={blue!80!black}
	}
% 	\usepackage[a4paper, total={7in, 10in}]{geometry}
% 	\allowdisplaybreaks
% 	\newcommand{\change}[1]{{\color{red}{#1}}}
\fi
%=================================================

==> New version Safety-aware BO - arXiv/notations.tex <==
% ------------------------------------------------
% transfer function ------------------------------
\newcommand{\Gp}{G_{\text{p}}} % Gp(s)
\newcommand{\Gv}{G_{\text{v}}} % Gv(s)
\newcommand{\Km}{K_{\text{m}}} % Km
\newcommand{\Kp}{K_{\text{p}}} % Kp
\newcommand{\Kv}{K_{\text{v}}} % Kv
\newcommand{\Ti}{T_{\text{i}}} % Ti
\newcommand{\Cp}{C_{\text{p}}} % Kp
\newcommand{\Cv}{C_{\text{v}}} % Kv

\newcommand{\pref}{{p}_{\text{ref}}} % reference position
\newcommand{\dotpref}{\dot{p}_{\text{ref}}} % reference velocity
\newcommand{\Ts}{T_{\text{s}}} % sampling time

% ------------------------------------------------
% Controller tuning: Grinding --------------------
\newcommand{\CSS}{C_\text{SS}} % steady state err at operation pt
\newcommand{\CSP}{C_\text{SP}} % overshoot at stopping pt
\newcommand{\CST}{C_\text{ST}} % overshoot at starting pt
\newcommand{\Ccrit}{C_\text{crit}} % overshoot at starting pt
\newcommand{\ut}{\underline{t}}
\newcommand{\ot}{\overline{t}}
\newcommand{\uk}{\underline{k}}
\newcommand{\ok}{\overline{k}}
\newcommand{\tSP}{t_\text{SP}} % time at stopping pt
\newcommand{\tST}{t_\text{ST}} % time at starting pt
\newcommand{\kSP}{k_\text{SP}} % time at stopping pt
\newcommand{\kST}{k_\text{ST}} % time at starting pt
% ------------------------------------------------
% Controller tuning: Generic ---------------------
\newcommand{\vcx}{\vc{x}}       % decision variable/controller gains
\newcommand{\nx}{n_{\vc{x}}}    % # of decision variable/controller gains
\newcommand{\es}{e}             % error signal

% ------------------------------------------------
% GP and GPR -------------------------------------
% \newcommand{\GP}[2]{{\mathcal{G}\!\mathcal{P}}(#1,#2)}
\newcommand{\GP}{{\mathcal{G}\!\mathcal{P}}}
\newcommand{\diag}{\mathrm{diag}}

% ------------------------------------------------
% CBO --------------------------------------------
\newcommand{\init}{{\text{init}}} % sampling time

\newcommand{\muf}{\mu^{\stiny{($f$)}}}
\newcommand{\mug}{\mu^{\stiny{($g$)}}}
\newcommand{\kf}{k^{\stiny{($f$)}}}
\newcommand{\kg}{k^{\stiny{($g$)}}}
\newcommand{\sigmaf}{\sigma^{\stiny{($f$)}}}
\newcommand{\sigmag}{\sigma^{\stiny{($g$)}}}
\newcommand{\nuf}{\nu^{\stiny{($f$)}}}
\newcommand{\nug}{\nu^{\stiny{($g$)}}}
\newcommand{\vckf}{\vc{k}^{\stiny{($f$)}}}
\newcommand{\vckg}{\vc{k}^{\stiny{($g$)}}}
\newcommand{\mxKf}{\mx{K}^{\stiny{($f$)}}}
\newcommand{\mxKg}{\mx{K}^{\stiny{($g$)}}}

\newcommand{\aEI}{a_\text{EI}} % acquisition function
\newcommand{\aCEI}{a_\text{CEI}} % acquisition function
\newcommand{\aEIf}{a^{\stiny{($f$)}}_\text{EI}} % acquisition function

% ------------------------------------------------
% ------------------------------------------------


==> New version Safety-aware BO - arXiv/sections/sec_00_abstr.tex <==
\begin{abstract} % Abstract of not more than 250 words.
%Cascade controller tuning is a time consuming process, that needs to be performed routinely upon maintenance.
This paper presents an automated, model-free, data-driven method for the safe tuning of PID cascade controller gains based on Bayesian optimization. The optimization objective is composed of data-driven performance metrics and modelled using Gaussian processes. We further introduce a data-driven constraint that captures the stability requirements from system data. Numerical evaluation shows that the proposed approach outperforms relay feedback autotuning and quickly converges to the global optimum, thanks to a tailored stopping criterion. We demonstrate the performance of the method in simulations and experiments. %on a linear axis drive of a grinding machine. %<---this part
For experimental implementation, in addition to the introduced safety constraint, we integrate a method for automatic detection of the critical gains and extend the optimization objective with a penalty depending on the proximity of the current candidate points to the critical gains. The resulting automated tuning method optimizes system performance while ensuring stability and standardization.


%The final achieved grinding performance is virtually identical to that corresponding to nominal tuning.


%The proposed method for automated and standardized tuning procedure achieves the same grinding performance as nominal tuning.




 %In addition, mechanical failures of the system are detected by the algorithm if their influence on the position or critical gains is significant.

\end{abstract}




==> New version Safety-aware BO - arXiv/sections/sec_01_intro.tex <==
\section{Introduction}

%Tuning of controller parameters enhances the corresponding system performance, prevents failures, and ensures robustness. Controllers of motion systems in industrial equipment are often tuned manually, which results in non-standardized performance. An efficient auto-tuning algorithm ensuring optimal performance and standardization of the controlled systems while maintaining safety and stability is essential, as re-tuning is regularly required.
%has to be performed regularly for industrial systems.
%violating safety constraints and requirements is thus 
%important and ensures 
%an important feature, as tuning has to be performed regularly, either for maintenance, or after servicing the components.
%This manual tuning process requires multiple iterations and good knowledge of the system.
% due to safety constraints in the equipment or to adaptations required in the standard automated tuning solutions
%. To enable repeatability, strict tuning protocols have to be followed, which is challenging due to gradual changes in the underlying mechanical components, variations, or simply due to faults.
To replace the cumbersome and often suboptimal manual controller tuning several auto-tuning methods have been proposed in the literature over the years. A comprehensive review of tuning methods for PID controllers, including mechatronics applications, is provided in \cite{borase2020review}.
Established auto-tuning methods such as relay feedback tuning \cite{Astrom} can be applied to a cascade PID control structure \cite{Hang3}. Global parameter optimization algorithms, e. g. particle swarm \cite{Kennedy}, ant colony \cite{Dorigo} or genetic algorithms \cite{Mitchell}, previously used for tuning in \cite{Solihin}, \cite{Chiha} and \cite{Zhang2006}, might be optimal for the system performance, but require the availability of a precise model of the plant, or a vast number of trials to find the optimum. 
%However, they are not guaranteed to fulfill all requirements in practice, may violate safety constraints by sending the system to its limits, and require one to open the outermost loop of the controller, which is not always feasible for industrial systems. 

 The general idea  of optimizing performance indicators derived from system data for tuning of control parameters has been explored through various approaches, e.g., iterative feedforward tuning \cite{Li2019,IterTuning_Li2018}, variable gain selection \cite{VarGain_Li2015}, data-driven feedforward learning \cite{FeedforLearning_Song2020}, constrained optimization using interior point barrier algorithms \cite{Constrained_Radac2013}. The performance criteria can be represented by features in the data measured during system operation at different values of the controller parameters \cite{Khosravi2020,Khosravi2020b}.
 %for the control of  semiconductor fabrication where high performance is of crucial importance \cite{Gao2013}. 
 
Stability and safety are important both in tuning and in operation, especially in industrial systems. The tuning of a cascade control system can be formulated as a data-driven optimization problem, where the objective is to find the best controller parameters that fulfill both performance criteria, and safety constraints. A data-efficient method for optimizing a priori unknown objective function is Bayesian optimization (BO), where the unknown objective function is often modelled as a Gaussian process (GP). The GP model uses available data from prior evaluations to provide a mean and uncertainty estimate of the underlying function at new input locations. The BO then uses the resulting estimate for selecting new inputs, based on the optimization of an acquisition function, which combines the uncertainty or information content at the inputs, and the corresponding predicted performance. 

Optimization constraints can be modelled as separate GPs \cite{Gardner}, and the inputs corresponding to fulfilling the constraints with high probability are chosen by adapting the acquisition function. The approach has been demonstrated for manufacturing processes \cite{Maier, MaierGrind2020}, and for the run-to-run control of reluctance actuators \cite{BOcontrolRun2020}. Another approach to respect safety constraints, known as safe Bayesian optimization (SafeOpt)   provides probabilistic guarantees that all candidate samples remain in the constraint set \cite{Sui}. SafeOpt has been implemented and verified for robotic applications  \cite{Berkenkamp,Berkenkamp2}, and for controller tuning in heat pumps \cite{Khosravi} and shown to enable automatic and safe optimization of controller parameters. It has been further extended by an adaptive discretization based on particle swarms by \cite{Duivenvoorden} to efficiently perform BO in high-dimensional parameters spaces. %One drawback of this approach is that the GP's kernel function needs very conservative length scales and therefore requires more evaluations for convergence. Moreover, SafeOpt requires initial points in all feasible sets, separated by constraints, to reliably find the global optimum.
% One drawback of this approach is that it requires more evaluations for convergence, to maintain safety, and also some domain knowledge of the plant and the expected regimes of operation, to ensure that the assumptions of the algorithm and the initial conditions are met. 

%, because the relationship between the gains and the cost is unknown and instability of the system, due to a poor choice of the gains, has to be avoided. Both can be achieved by constrained Bayesian optimization. Furthermore the result of the algorithm is optimal in terms of a defined cost function, in comparison to other more simple auto-tuning methods, like relay feedback tuning and the algorithm itself is more data efficient than e.g. grid search, particle swarm optimization or SafeOpt.

 Controller tuning via BO is a suitable method to maximize the performance of industrial positioning systems by optimizing a combination of performance features \cite{Khosravi2020b}. However, when a system is embedded in a more complex equipment, additional forces might be applied in operation, or the system can be subject to wear, and the aspect of stability and safety gains priority. In this paper, we propose a safe, data-driven, model-free approach for the tuning of cascade controllers. The main contributions of the paper are: 1) We propose a safety-aware performance-based tuning algorithm, where safety and stability are ensured by informing the algorithm of the experimentally determined unsafe controller parameters; 2) The algorithm finds controller parameters with maximal performance; 3) We validate the approach numerically against benchmark safe tuning methods, and experimentally, on a linear axis component of a computer numerical control (CNC) grinding machine.

%we propose a data-driven, model-free approach to tune controllers where the simultaneous tuning of parameters in nested loops is beneficial while ensuring stability in the system by informing the algorithm of the experimentally determined unsafe controller parameters. The main contributions of the paper are: 1) We demonstrate an efficient performance-based tuning algorithm, which ensures maximal performance without changing the structure of the underlying controller; 2) We guarantee safe and stable operation by introducing both a constraint and a penalizing term in the optimization objective, ensuring that the controller parameters are sufficiently far from critical gains at each iteration.
%3) We validate the approach numerically against benchmark tuning methods; %(relay feedback tuning and safe Bayesian Optimization); 
 % which is an example of computer numerical control (CNC) system.

% Contributions: 1) introducing the algorithm, 2) numerical evaluation and proof for outperforming benchmark methods, 3) More practical data-driven term for improving the safety by informing the cost, 4) experimental evaluations

We first present the safety-aware tuning problem in section \ref{sec:PF}, then we describe the proposed approach for safe tuning in \ref{sec:BO}. The system modeling, performance metrics, and numerical implementation and verification of the algorithm are provided in section \ref{sec_model}, \ref{sec_BO}, and \ref{sec_simulation_1}, respectively. Section \ref{sec_experiments} presents the safety-aware tuning approach implemented on the experimental system. 



%derive and discuss the model of the testbed system in Section \ref{sec_model}, and  we introduce the proposed tuning scheme in Section \ref{sec_BO}.
%In section \ref{sec_model} a model of the system is introduced, derived from first principles in combination with system identification techniques, in section \ref{sec_BO} \cmb{some preliminaries for GPs, BO,} and the introduced algorithm are provided. 
%Section \ref{sec_simulation} presents numerical results, comparing the constrained Bayesian optimization tuning with relay feedback auto-tuning and the SafeOpt Bayesian optimization algorithm, and 



==> New version Safety-aware BO - arXiv/sections/sec_02_PF_01.tex <==
\section{Safety-Aware Controller Tuning Problem}
\label{sec:PF} % problem formulation
Consider a closed-loop system designed for controlling a possibly nonlinear plant.  Let $\vc{x}\in\Xbb$ be the vector of parameters describing the controller in the loop, where $\Xbb\subseteq\Rbb^{\nx}$ is the set of admissible controller parameters. These parameters should be designed such that the overall closed-loop performance is optimized and meanwhile the safety of the system is preserved. Based on the tracking error signal, i.e., the difference between the reference signal and the output signal, one can introduce various metrics indicating the quality of tracking, e.g., the magnitude of overshoot, the settling time, the steady-state error, the rising time, and other similar quantities. Given the reference signal and a fixed control structure, the error signal depends mainly on the vector of parameters $\vcx$. Accordingly, each of the above performance metrics is a function of $\vc{x}$, and hence, we denote them by $c_i:\Xbb\to\Rbb$, for $i=1,\ldots,n_\vc{c}$.
The overall performance metric, $f:\Xbb\to\Rbb$,  is defined as a weighted sum of the separate performance metrics, i.e., 
\begin{equation}\label{eqn:overall_perf}
f(\vcx):=\vc{w}^\tr \vc{c}(\vcx) = \sum_{i=1}^{n_{\vc{c}}}w_i c_i(\vcx),\qquad \vcx\in\Xbb,    
\end{equation}
where $\vc{c}(\vcx):=[c_i(\vcx)]_{i=1}^{n_{\vc{c}}}$ and $\vc{w}:=[w_i]_{i=1}^{n_{\vc{c}}}$.
The weights $w_1,\ldots,w_{n_{\vc{c}}}$ are decided based on the importance and the scale of the corresponding performance metric.
Similarly, one can consider a safety metric, $g:\Xbb\to\Rbb$, indicating the margin of the safety for a choice of controller parameters. For example, $g(\vcx)$ can be the overshoot observed in the response of the system.
Given the introduced metrics for performance and safety, we can introduce the 
\emph{safety-aware controller tuning problem}.
More precisely, to obtain the optimal controller gains $\vcx^*$ and meanwhile preserve the safety, we need to solve the following optimization problem
\begin{equation}\label{eqn:CBO}
\begin{array}{cl}    
\minOp_{x \in \Xbb}
&
f(\vcx)= 
\vc{w}^\tr \vc{c}(\vcx)
\\\text{s.t.}
&
g(\vcx) \leq g_{\text{tr}}\,, 
\end{array}
\end{equation}
where $g_{\text{tr}}$ is a safety threshold. 
For further safety improvement, one can consider additional performance metrics as barrier functions penalizing parameters close to critical gains.


The performance objective function $f$ and the safety constraint $g$ cannot be analytically calculated, i.e., they 
do not have a tractable closed-form expression, even when the dynamics of system are known. 
Indeed, with respect to each controller parameters, $\vc{x}$, 
one should perform an experiment on the system, measure the tracking error signal, and subsequently, calculate the value of $f(\vcx)$ and $g(\vcx)$.
In other words, each of these functions is given in a {\em black-box oracle} form.
Therefore, for tuning the controller gains via \eqref{eqn:CBO}, we utilize constrained Bayesian optimization (CBO), a data-driven approach for solving optimization problems whose objective function and constraints are available as expensive to evaluate black-box functions.
Accordingly, we have a data-driven tuning method which optimizes the closed-loop performance and preserves the safety of system (see Figure \ref{fig:scheme}).  
Note that this methodology can be extended to the control loop with multiple feedforward and feedback branches.

\begin{figure}[t]
\centering
\includegraphics[width = 0.485\textwidth]{Figs/BLK_Diagram_01.pdf}%    
\caption{The safety-aware performance-based controller tuning scheme.}
\label{fig:scheme}
%\vspace{-5mm}
\end{figure}


==> New version Safety-aware BO - arXiv/sections/sec_03_CBO_01.tex <==
\section{Safe Controller Tuning Using Constrained Bayesian optimization}
\label{sec:BO}
The constrained Bayesian optimization (CBO) approach is based on sampling from the space of decision variables, $\Xbb$, and performing experiments. The scheme of controller tuning procedure based on this is shown in Figure  \ref{fig:scheme}. The detailed implementation is summarized in Algorithm \ref{alg:safety_aware_tuning} and explained in the following.


%The constrained Bayesian optimization samples and learns both the objective function and the constraints online, and finds the global optimum iteratively \cite{Mockus, Gardner}, using Gaussian process regression to build a surrogate for the objective and the constraints, and to quantify the uncertainty.
Assume that initially we are given a collection of controller gains  
%\begin{equation}\label{eqn:X_init}
$\Xbb_{\init}:= \{\vcx_i\in\Xbb\ \! |\ \! i=1,\ldots,m_\init\}$.
% be an initial set of controller gains. 
%where with respect to each $\vcx_i\in \Xbb_{\text{init}}$ an experiment is performed and subsequently, we have evaluated the  performance metric and the constraint in \eqref{eqn:CBO}, respectively denoted by $y_i$ and $z_i$.
%The optimization process is summarised in Algorithm \ref{alg:safety_aware_tuning}. 
The algorithm maintains a pool of data $\Dcal_m:=\{(\vcx_i,y_i,z_i)\ \!|\ \! i=1,\ldots,m\}$,
where $\vcx_i$ are controller gains for which experiments have been performed, and, $y_i$ and $z_i$ are respectively the values of $f(\vcx_i)$ and $g(\vcx_i)$ computed from data collected in these experiments, i.e., the error signal. To capture uncertainty in the data collecting process we assume that $y_i=f(\vcx_i)+n_i$ and $z_i=g(\vcx_i)+\delta_i$, for all $i$,  where $n_i$ and $\delta_i$ are noise realisations. We assume that initially there are already $m\ge m_\init$ data points from the earlier operation of the machine and initialise $m=m_\init$. At each step of the algorithm 
%Indeed, we have $y_i=f(\vcx_i)+n_i$ and $z_i=g(\vcx_i)+e_i$, for any $i$, where $n_i$ and $e_i$ are introduced for capturing the potential uncertainties in the evaluations. 
%Given data set $\Dcal_m:=\{(\vcx_i,y_i,z_i)\ \!|\ \! i=1,\ldots,m\}$, where $m\ge m_\init$,
we can perform a Gaussian process regression (GPR) for building surrogate functions for the performance metric and the constraint, denoted respectively by $f_m$ and $g_m$. 
More precisely, let $\GP(\muf,\kf)$ and $\GP(\mug,\kg)$ be Gaussian process priors respectively for $f$ and $g$, where $\muf:\Xbb\to\Rbb$ and $\kf:\Xbb\times\Xbb\to\Rbb$ are the mean and kernel functions in the GP prior taken for $f$, and similarly, $\mug:\Xbb\to\Rbb$ and $\kg:\Xbb\times\Xbb\to\Rbb$ are the mean and kernel functions in the GP prior taken for $g$.
%Given the set of data $\Dcal_m$ and the priors for $f$ and $g$, using the Bayes rule for the conditional probability, we can predict the value of these functions at each vector of controller gains $\vcx\in\Xbb$.
Let the information matrices $\mx{X}_m$ and $\vc{y}_m$ be defined respectively as
$\mx{X}_m:=[\vcx_1,\ldots,\vcx_m]^\tr$, 
and 
$\vc{y}_m:=[y_1,\ldots,y_m]^\tr$. 
Then, we have $f_m(\vcx)\sim\Ncal\left(\muf_m(\vcx),\nuf_m(\vcx)\right)$, where the mean and variance are characterized as follows
\begin{align}
\label{eqn:post_fm}
\muf_{m}(\vcx) & := 
\muf(\vcx) \notag
\\&\quad\ \  + 
\vckf_{m}(\vc{x})^\tr 
(\mxKf_{m} + \sigma_{n}^{2}\eye)^{-1} 
(\vc{y}_m - \muf(\mx{X}_m)),  
\\ \label{eqn:cov}
\nuf_{m}(\vcx) &:=
\kf(\vcx,\vcx)
-
\vckf_{m}(\vc{x})^\tr  
(\mxKf_{m} + \sigma_{n}^{2}\eye)^{-1} 
\vckf_{m}(\vc{x}), 
\end{align}
where
% $\vckf_{m}(\vc{x}) :=
% [\kf(\vcx,\vcx_1),\ldots,\kf(\vcx,\vcx_m)]^\tr$ and $
% \muf(\mx{X}_m) :=
% [\muf(\vcx_1),\ldots,\muf(\vcx_m)]^\tr$,
%\begin{equation}
%\begin{split}
the vector $\vckf_{m}(\vc{x}) = [\kf(\vcx,\vcx_1),\ldots,\kf(\vcx,\vcx_m)]^\tr$ , the vector
$\muf(\mx{X}_m) =
[\muf(\vcx_1),\ldots,\muf(\vcx_m)]^\tr,$
%\end{split}
%\end{equation}
matrix  $\mxKf_{m}$ is defined as $[\kf(\vcx_i,\vcx_j)]_{i,j=1}^m$, $\eye$ is the identity matrix and $\sigma_n^2$ is the variance of the uncertainty in the evaluations of performance metric. 
Similarly, we have 
$g_m(\vcx)\sim\Ncal\left(\mug_m(\vcx),\nug_m(\vcx)\right)$
where the mean $\mug_m(\vcx)$ and variance $\nug_m(\vcx)$ are defined as in the previous case.

Given these probabilistic surrogate models for the performance metric and constraint, we can decide on the next candidate  sampling point, $\vcx_{m+1}\in\Xbb$, for the controller gains to be used in the next experiment. 
% and subsequent evaluation of the performance metric and constraint.
% To this end, using these GP models, one can consider a suitable \emph{acquisition function} as the sampling criterion resulting in exploration of the regions of the domain $\Xbb$ with the highest prediction uncertainty and exploitation of the points of $\Xbb$ with the lowest predicted cost, and meanwhile, satisfying the safety constraint with high probability \cite{Frazier}.
Using these GP models, one can consider an appropriate \emph{acquisition function} as the safe sampling criterion resulting in a suitable exploration-exploitation trade-off, (exploration of the regions of domain $\Xbb$ with the highest prediction uncertainty and exploitation of the points of $\Xbb$ with the lowest predicted cost), satisfying the safety constraint with high probability \cite{Frazier}.
 Let the \emph{expected improvement} function, $a_{\text{EI},m}:\Xbb\to \Rbb$, be defined as
% \begin{equation}\label{eq:EI}
% \!\!
% a_{\text{EI},m}(\vcx)
% \!:=\!
% (\muf_m(\vcx)\!-\!\vc{y}_m^+) \Phi(\xi_m(\vcx))
% +
% (\nuf_m(\vcx))^{\frac{1}{2}} \varphi(\xi_m(\vcx)), 
% \!\!
% \end{equation}
\begin{equation}\label{eq:EI}
a_{\text{EI},m}(\vcx)
:=
\Big{(}\xi_m(\vcx)\Phi(\xi_m(\vcx))
+
\varphi(\xi_m(\vcx))\Big{)}\ \! \nuf_m(\vcx)^{\frac{1}{2}}, 
\end{equation}
where 
$\Phi$ and $\varphi$ are respectively the cumulative distribution function and probability density function of the standard normal distribution, and $\xi_m(\vcx):=(\muf_m(\vcx)-\vc{y}_m^+)/\nuf_m(\vcx)^{\frac{1}{2}}$ given that $\vc{y}_m^+$ is the best observed performance amongst the first $m$ experiments. 
Note that when the optimization problem is unconstrained, one can use $a_\text{EI,m}$ as the acquisition function  
aiming for a vector of controller gains with highest expected improvement of the performance metric $f$ \cite{Gardner}.
To include the constraint in \eqref{eqn:CBO}, one needs   to include the feasibility probability of the candidate sample. %for the controller gain. 
This results in %an acquisition function $a_{\text{CEI},m}:\Xbb\to \Rbb$, which is called 
 the \emph{constrained expected improvement}  \cite{Gardner},  defined as
\begin{equation}\label{eq:CEI}
a_\text{CEI,m}(\vcx)=  
\Phi\left(
\frac{g_{\text{tr}}-\mug_m(\vcx)}{\nug_m(\vcx)^{\frac{1}{2}}}\right)
a_\text{EI,m}(\vcx).
\end{equation} 
Subsequently, the next sampling point is obtained as 
\begin{equation}\label{eqn:x_next}
    \vcx_{m+1} := \argmax_{\vcx\in\Xbb}\ \! a_\text{CEI,m}(\vcx).   
\end{equation}
In order to solve optimization problem \eqref{eqn:x_next}, one can utilize various methods. 
% such as particle swarm optimization.
Given $\vcx_{m+1}$, a new experiment is performed, the performance $y_{m+1}$ and constraint $z_{m+1}$ are evaluated, and the set of data is updated to $\Dcal_{m+1} = \Dcal_m \cup\{(\vcx_{m+1},y_m,z_m)\}$.
The sequence $\vcx_1,\vcx_2,\vcx_3,\ldots$ generated by this iterative procedure converges to the solution of \eqref{eqn:CBO} in a suitable sense \cite{Gardner}.

For the practical implementation of the controller tuning procedure, we need a stopping condition to ensure timely termination of the optimization algorithm. The stopping criterion can be based on the  maximal number of iterations, repeated sampling in the region of the minimal cost observed \cite{Khosravi2020b}, a threshold on the expected improvement acquisition function \cite{Nguyen}, or the convergence status of the uncertainty in the GP model of the cost \cite{Maier}. %While \cite{Nguyen} proposes a lower bound threshold of the expected improvement acquisition function as termination criterion,
The stopping criterion used here depends on 
%the maximum of the acquisition function on the past iterations, where 
the ratio between the current expected improvement and the maximal expected improvement over all the previous iterations. 
This improves the robustness of the stopping condition with respect to the variation 
%in $a_{\text{CEI}}$, due to the dependence on 
of the GP model hyperparameters. 
More precisely, the stopping condition is met when for three consecutive iterations we have
\begin{equation}
\label{eq:stop_aCEI}
a_\text{CEI}(\vcx_m) \leq \eta_\text{limit}\ \!\max_{0\leq i \leq m-1}a_\text{CEI}(\vcx_i),    
\end{equation}
where $\eta_\text{limit} \in [0,1)$
is a pre-determined threshold. 
The condition stops the iterative sampling procedure when the expected improvement does not change significantly by further exploration. 
% The iteration index at which the algorithm stops is denoted by $m^*$.
The stopping iteration index is denoted by $m^*$.

The initial set of data $\Dcal_{m_{\init}}$ as well as the choice of kernel functions $\kf$ and $\kg$ play a significant role in the performance of the scheme.
Here to have maximally informative data set $\Dcal_{m_{\init}}$, initial sampling points $\Xbb_{\init}$ are drawn from a Latin hyper-cube experimental design \cite{mckay2000comparison}.
Subsequently, the hyperparameters of kernels $\kf,\kg$ 
are updated by minimizing the negative log marginal likelihood \cite{Rasmussen}, and kept fixed during the rest of the controller tuning procedure.
Though tuning the hyperparameters at every iteration might provide better GP models, it can disturb the convergence of the scheme.
While various options for the choice of kernel are introduced in the literature \cite{Rasmussen}; here 
we employ Matern kernels with parameter $\nu=\frac{3}{2}$ and automatic relevance determination, which enables the use of different kernel length scale parameters for each dimension of the input data \cite{Rasmussen}. 
Regarding the mean functions, we set $\muf=0$ and $\mug=0$ \cite{Rasmussen}. Note that one may employ other options 
when there is a prior knowledge on the structure of $f$ and $g$  \cite{Rasmussen}.

%The complete scheme of the proposed controller tuning approach is summarized in Algorithm \ref{alg:safety_aware_tuning}. 

\begin{algorithm}[t]%------------------------
\caption{Safety-Aware Controller Tuning Method}\label{alg:safety_aware_tuning}
\begin{algorithmic}[1]
\State \textbf{Input:} Set $\Xbb$, training data set $\Dcal_{m_\init}$, weight vector $\vc{w}$, GP priors $\GP(0,\kf)$ and $\GP(0,\kg)$, and  $\eta_\text{limit}$.  
\State Using $\Dcal_{m_\init}$ estimate the vectors of hyperparameters for $\GP(0,\kf)$ and $\GP(0,\kg)$, by minimizing the negative log marginal likelihood function.
\State $\Dcal_{m-1} = \Dcal_{m_\init}$ and $m-1= m_\init$.
\While{stopping condition is not met}
\State Derive $\vc{x}_{m}$ by solving \eqref{eqn:x_next}.
\State Set controller gains to $\vc{x}_{m+1}$, run the  experiment and measure the error signal $e^{(m)}$.
\State Obtain the values of the performance and the constraint functions $y_{m}$ and $z_{m}$ by calculating $c_i(\vcx)$, for $i=1,\ldots,n_{\vc{c}}$, and $g(\vcx)$.
\State Update the GP models: calculate $\muf_m,\nuf_m$ and $\mug_m,\nug_m$ (see \eqref{eqn:post_fm} and \eqref{eqn:cov}).
\State Update set of data: $\Dcal_m =  \Dcal_{m-1}\cup \{(\vcx_{m},y_{m},z_{m})\}$.
\EndWhile\label{DCP_loop}
\State \textbf{end} 
\State \textbf{Output:} $\vc{x}_{m^*}$.
\end{algorithmic}%%%\vspace{-2mm}
\end{algorithm}%%\vspace{-3mm}
%\vspace{-2mm}

==> New version Safety-aware BO - arXiv/sections/sec_04_NumVer_01.tex <==

%%\vspace{-3mm}
\section{Numerical Verification on a  CNC %Grinding 
Machine}
%In this section, we introduce the test bed system for the proposed method.
%Also, we derive the mathematical model of the system and the implemented control scheme to be utilized later for the numerical evaluations.
%The system and the control structure are described in section \ref{sec_model_1}. A model of the nonlinear force ripple and cogging force and the linear dynamics is developed in sections \ref{sec_model_2} and \ref{sec_model_3} and its parameters are identified and validated with measurement data. 
%\subsection{System model and Control Structure}
%\label{sec_model_1} 
% we don't have another subsection.
The system of interest is a linear axis drive integrated in a four axis CNC grinding machine, endowed with two perpendicular linear axes moving the grinding wheel, and two rotational axes for the movement of a fixed work-piece  (See Figure \ref{fig:machine_axes}). 
Each axes is driven by a controlled brushless permanent magnet AC motor. 
The corresponding controllers are tuned independently in a special operational mode which does not involve grinding. %\cmr{since we are removing section on tuning during grinding should we keep this sentence?}. 
The parameters of the controllers should be tuned to ensure adequate performance of the closed loop system. %, given that the load of the system may change during grinding operation. 
%\cmm{Should we put back the grinding quality results?} 
In this work, we are mainly focused on the linear axes $\mathrm{X}$ and $\mathrm{Y}$ for moving the grinding wheel in the direction perpendicular to the ground surface,  due to its critical impact on the grinding quality. We report the tuning of the $\mathrm{X}$-axis controller, although we implemented the method also for the $\mathrm{Y}$-  and for the rotational $\mathrm{B}$- axis with similar results.
The same method can be applied to other axes in the grinding machine.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{Figs/setup.pdf}
    \caption{Left: The sketch of the linear $\mathrm{X, Y}$- and rotational $\mathrm{A, B, C}$- axis with respect to the grinding wheel. Right: The actual grinding machine.}
    \label{fig:machine_axes}
    %\vspace{-5mm}
\end{figure}

%=================================================
%\vspace{-1mm}
\subsection{System Structure and Modelling}
\label{sec_model}

%\subsection{System Model and Control Structure}
The plant is modeled as a combination of a linear sub-system and a nonlinear sub-system, as shown in Figure \ref{fig:Control_Structure}. 
The linear block models the linear axis as a damped single mass system, following \cite{Khosravi2020}, 
with transfer function $G(s)$ defined as 
$G(s) = \begin{bmatrix}
\Gp(s)&\Gv(s)
\end{bmatrix}^\tr$,
% \begin{equation}\label{eqn:Gs}
% G(s) 
% :=
% \begin{bmatrix}
% \Gp(s)\\\Gv(s)
% \end{bmatrix}    
% =
% \begin{bmatrix}
% \frac{1}{ms^2 + bs}\\\frac{1}{ms + b}
% \end{bmatrix},    
% \end{equation}
% \begin{align*}
% \Gp(s) = \frac{\Km}{ms^2 + bs}\, , \quad
% \Gv(s) = \frac{\Km}{ms + b}\, ,
% \end{align*}
% \begin{align*}
% \Gp(s) = \frac{1}{ms^2 + bs}\, , \quad
% \Gv(s) = \frac{1}{ms + b}\, ,
% \end{align*}
where $\Gp(s)$ and $\Gv(s)$ are the transfer functions respectively from force to position and from force to velocity. %$\Km$ \cmm{is the force induced by the motor operating at full power}, 
These transfer functions mainly depend on the mass of the axis, $m$, and also the damping coefficient $b$ due to the friction. 
These values are estimated using a least squares fitting identification procedure and provided in Table \ref{tab:ForceRipple}. 
%The transfer functions of the linear dynamics are discretized with the sampling time of the measurement. <----not necessary at this point!!!
\iffalse
\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{Figs/BlockDiagram_Gs_03.pdf}
\caption{The block-diagram of the plant}
\label{fig:plant}
\end{figure}
\fi
The nonlinear subsystem models the nonlinear phenomena of force ripple and cogging effects in the permanent magnet motor.
Force ripple is caused by the irregularity of the magnetic field of the permanent magnet and the inaccuracy of the electronic communication by the servo amplifiers \cite{Rohrig}, while the cogging force results from the attraction between the ferromagnetic core of the motor windings and the permanent magnets on the rail \cite{Villegas}. 
These forces depend on the position with an almost periodic behaviour. Following \cite{Rohrig}, we model them by Fourier truncated expansion:
% \begin{equation}\label{eq:Force_Ripple_new}
% f_\vc{c}(p) = c_1 + c_2p +  
% \sum_{k=1}^{n} c_{2 k+2}\!\ \sin\!\Big{(}\frac{2 k \pi}{c_{3}}(p+c_{2 k+3})\Big{)}\, , \end{equation}
\begin{equation}\label{eq:Force_Ripple_new}
f_\vc{c}(p) = c_1 + c_2p +  
\sum_{k=1}^{n} c_{2 k+2}\!\ \sin\!\Big{(}\frac{1}{c_{3}}2 k \pi p+c_{2 k+3}\Big{)}\, , \end{equation}
where $p$ is the position, $c_1$ is the average thrust force, $c_2$ is the gradient of the curve caused by sealing bellows, $c_3$ is the largest dominant period  described by the distance of a pair of magnets in the rail, $n$ is the number of modelled frequencies, and, $c_{2k+2}$ and $c_{2k+3}$ are respectively the amplitudes and the phase shifts of the sinusoidal functions, for $k=1, 2,\ldots,n$. 
The vector of parameters 
$\vc{c}:=[c_1,\ldots,c_{2n+3}]^\tr$
%$\{c_k\ |\ k=1,\ldots,2n+3\}$ 
%%in \eqref{eq:Force_Ripple_new} 
are estimated using least squares error minimization between the modelled ripple and cogging forces in \eqref{eq:Force_Ripple_new} and the measured force signal at constant, non-zero velocity (to cancel the effects from linear dynamics). The estimated values of the parameters are provided in Table \ref{tab:ForceRipple}.  In our case, a single harmonic suffices to capture most of the nonlinearity present in the system.
%As it is shown in Figure \ref{fig:Plant}, the nonlinear effects of the force ripple and cogging force are introduced as an additional signal depending on the position feedback value.
\begin{table}[b]%\vspace{-2mm}
 \caption{Parameters of the system}% Cogging force and system dynamics parameters
 \label{tab:ForceRipple}
    \centering
    \ra{1.1}
    \begin{tabular}{ @{}l l l @{} }
    \toprule
     Parameter & Value & Unit\\
     \midrule
    %\textbf{Cogging Parameters} &   \\
    $n$ number of frequencies & $1$ &-\\
    %$c_0$ offset in force & 78.82& N\\
    $c_1$ average thrust force & -$104.9$& N\\
    $c_2$ gradient & $682.44$ & N/m\\
    $c_3$ distance of pair of magnets& $2.364\text{e-}1$&m\\
    $c_4$ amplitude & $23.55$&N\\
    % $c_5$  phase shift& $3.3\text{e-}8$&m\\ 
    $c_5$  phase shift& $8.77\text{e-}7$&m\\ 
    %\textbf{Dynamics Parameters} & \\
%    $\Km$ unit translation of the motor & $14.1$ & $\mathrm{\frac{N}{[\% \, motor \, power]}}$\\
    $m$ axis mass & $388.61$ & kg\\
    $b$ damping coefficient  & $2224.60$ &kg/s\\
    \bottomrule
    \end{tabular}
\end{table} 

\begin{figure}[h]
\centering
\includegraphics[width=0.485\textwidth]{Figs/ControlDiagram_CL_all_01}
\caption{The plant and the control structure of the linear axis.}
\label{fig:Control_Structure}
%\vspace{-5mm}
\end{figure}
The linear axis is controlled by a three-level cascade controller shown in Figure \ref{fig:Control_Structure}. 
The outermost loop controls the position by P-controller $\Cp(s)=\Kp$, and the middle loop controls the velocity by PI-controller $\Cv(s) = \Kv(1+\frac{1}{\Ti s})$. 
The innermost loop of the control structure is a current controller for the permanent magnet AC motor of the linear drive, which is pre-tuned robustly and hence treated as a part of the plant $G(s)$.  
% The innermost loop of the control structure is a current controller for the permanent magnet AC motor of the linear drive. This feedback PI-controller is well tuned, and hence, we treat it as a part of the plant $G(s)$. 
As illustrated in Figure \ref{fig:Control_Structure},
feedforward structures are used to accelerate the response of the system. 
Similar to the current controller, the gains in these feedforward blocks are set initially and not modified during the tuning procedure.
Accordingly, in the followings, we consider two cases for the controller parameters to be tuned:  $\mathrm{x} = (\Kp, \Kv, \Ti)$ and $\mathrm{x} = (\Kp, \Kv)$, where in the latter one $\Ti)$ is set to $\Ti= 7.5$ms.
% Since this is a very stable feedback PI-controller, its parameters do not have to be re-tuned for maintenance purposes and it is treated as part of the plant $G(s)$. 
% The remaining two control loops are inner velocity feedback loop $\Cv(s)$, controlled by a PI-controller, and the outer position feedback loop $\Cp(s)$, controlled by a P-controller: 
% \begin{align}
% \Cp(s)=\Kp, \quad \Cv(s)=\Kv(1+\frac{1}{\Ti s}) \, .
% \label{eq:Controller_TF}
% \end{align}
%Filters altering the force feedforward signal and the position controller output can be \cmm{(``can be" or ``are")} added to the structure to suppress resonant frequencies. 

\begin{comment}
\begin{table}[b]
\caption{Control system limitations}
\centering
 \begin{tabular}{||c c c c||} 
 \hline
     & $p_r$ [mm or °] & $v_r$/$v_{ff}$ [mm/s or U/min] & $F_r$/$F_{ff}$ [\% motor power]\\ [0.5ex] 
 \hline\hline
 GX & 94 -- 231 & -315 -- 315 & -400 -- 400\\ 
 \hline
\end{tabular}
\label{tab:CS_limits}
\end{table}
\end{comment}

%and moreover the internal auto-tuning method by the BOSCH Rexroth controller, based on step responses of the velocity reference value, has shown difficulties coping with this emergency stop automatism, while producing unsatisfying low gains for the controller, when functioning. 

%\subsection{Modeling of nonlinear effects}
%\label{sec_model_2}
%One of the main challenges in modelling permanent magnet motors is the presence of nonlinear force ripple- and cogging effects. While force ripple is caused by the irregularity of the permanent magnets' magnetic field and inaccuracy of the electronic communication by the servo amplifiers \cite{Rohrig}, the cogging force results from the attraction between the ferromagnetic core of the motor windings and the permanent magnets on the rail \cite{Villegas}. Both forces are dependent on the position and are represented by periodic functions, while the force ripple is also dependent on the voltage signal of the servo amplifier input. Because the tuning of the grinding machine is done without load and at the same speed (e.g. 30mm/s for GX), the dependency of the force ripple on the servo amplifier input can be neglected for this work. Thus, both effects can be described together, using Fourier decomposition:
%\begin{align}
%\label{eq:Force_Ripple_new}
%&F(x,c)=c_{0}\ \!\mathrm{sign}(\dot{x}_{r})+c_{1}+c_{2}x~+  \\
%&+\sum_{k=0}^{M-1} c_{2 k+4} \sin \left(\frac{2 %\pi(k+1)}{c_{3}}\left(x+c_{2 k+5}\right)\right)\, , \nonumber 
%\end{align}
%where $x$, $x_r$ are the position and position reference, respectively, $c_{0}$ is the coefficient describing the offset in force caused by overcoming the friction, $c_1$ is the average thrust force, $c_2$ is the gradient of the curve, caused by sealing bellows, $c_3$ is the highest dominant period, described by the distance of a pair of magnets in the rail, $c_{2k+4}$ are the amplitudes of the sinusoids, $c_{2k+5}$ are the phase shifts of the sinusoids and $M$ is the number of modelled frequencies. The nonlinear effects of the force ripple and cogging force are introduced as an additional signal depending on the position feedback value.
%, (see $F_c(p)$ illustrated in figure \ref{fig:Plant}), where the plant G of figure \ref{fig:Control_Structure} is shown in more detail.
% \begin{figure}[H]
% \centering
% \includegraphics[width=0.4\textwidth]{img/Plant.pdf}
% \caption{Complete plant model of the system \cmr{[Mohammad: I will redo this block-diagram. It can be done nicer \Coffeecup \Smiley \ManFace.]}}
% \label{fig:Plant}
% \end{figure}
%The parameters $c_i$ of \eqref{eq:Force_Ripple_new} are identified by a least squares error minimization between the modelled force ripple and cogging force and the measured force signal at constant, non-zero velocity (to cancel the effects from linear dynamics). The identified parameters are provided in table \ref{tab:ForceRipple}. 
\iffalse
\subsection{Parameter Estimation}%Dynamics parameters identification}
\label{sec_model_3}
In order to estimate the parameters 

As a next step the linear dynamics is identified. In figure \ref{fig:plant} this is illustrated by the linear transfer function $G(s)$. The position, velocity and force of a closed loop trapezoidal tuning picture are measured at 0.5ms sampling time and a velocity of 30mm/s. The force measurement is then corrected by subtraction of the cogging and force ripple effects and elimination of the static friction force (setting the force to zero, when the velocity is close to zero). The corrected force measurement is then used as input, and the position and velocity measurements as outputs in a least squares minimization fitting procedure. \cmr{(numerical values for fitting error? If we have them and if they are nice \Smiley maybe we should use them like 85\% R-square and validation 75\% R-square..., otherwise the reviewer will ask for it...!!!)}
We validated the complete controller and plant model with an additional set of measurements of the position error and the force signal.

%As a next step the linear dynamics is identified. In figure \ref{fig:plant} this is illustrated by the linear transfer function $G(s)$. The position, velocity and force of a closed loop trapezoidal tuning picture are measured at 0.5ms sampling time and a velocity of 30mm/s. The force measurement is then corrected by subtraction of the cogging and force ripple effects and elimination of the static friction force (setting the force to zero, when the velocity is close to zero). The corrected force measurement is then used as input, and the position and velocity measurements as outputs in a least squares minimization fitting procedure.

%, to identify the parameters in the following damped single mass system's transfer functions 
%$G_p(s) = \frac{K_m}{ms^2 + bs}$ and
%$G_v(s) = \frac{K_m}{ms + b}$, following \cite{Khosravi2020}. Here $G_p(s)$ and $G_v(s)$ are the force to position and force to velocity transfer functions, respectively, $K_m$, $m$ and $b$ are a unit translation, the axis' mass and the damping coefficient, caused by friction. The identifed values of $K_m$, $m$ and $b$ are provided in table \ref{tab:ForceRipple}. The transfer functions of the linear dynamics are discretized with the sampling time of the measurement. 



%%The nominal controller settings used in the model and in the real system for the position P and velocity PI controller are ($K_\text{p}^\text{nom}$ = 20$\mathrm{\frac{1000}{min}}$, $K_\text{v}^\text{nom}$ = 1$\mathrm{\frac{N}{mm/min}}$, $T_\text{i}^\text{nom}$ = 7.5ms). 
%\begin{figure}[H]
%\centering
%  \includegraphics[width=0.35\textwidth]{img/GX_Lsqfit_validation_F_posError.pdf}
%\caption{\cmr{We can also remove this figure. }Least squares fit validation}
%\label{fig:Lsqfit_val_GX}
%\end{figure}
\fi


%The position reference is fed as input to the closed loop system, and the position error and the force signal corresponding to measurement and simulation are compared (see figure \ref{fig:Lsqfit_val_GX}).
 
%To validate the complete model of the cascade control structure and the plant, the closed loop system is rebuilt in MATLAB Simulink and validated with an additional set of measurements. Both the measurement and the simulation use the nominal controller settings for the position P and velocity PI controller ($K_{p}`\text{nom}$ = 20$\mathrm{\frac{1000}{min}}$, $K_{v}`\text{nom}$ = 1$\mathrm{\frac{N}{mm/min}}$, $T_{inom}$ = 7.5ms). The position reference is fed as input to the closed loop system, and the position error and the force signal corresponding to measurement and simulation are compared (see figure \ref{fig:Lsqfit_val_GX}). 


%================================================
%================================================
%================================================
%================================================
%\vspace{-2mm}
\subsection{Safe Controller Tuning for the CNC Machine}
\label{sec_BO}
% decision variables, operation & performance
% black-box functions: objective + constraints
% Bayesian optimization: GPR + sampling for exploration/exploitation
% historical data + regression based on MAP -> surrogate function + uncertainty quantification
% sampling based on maximum improvement and 

%In the tuning problem, the decision variable, denoted by $\vcx$, is the vector of controller gains. 
%Here, we consider two cases $\vcx = (\Kp,\Kv,\Ti)$ and $\vcx = (\Kp,\Kv)$, where in the latter one $\Ti$ is set to $\Ti = 7.5$ms.
During standard operation, the grinding machine moves back and forth, starting from a reset point, moving towards the operation location, remaining there to perform the grinding mission, and then returning to the setback point.
Accordingly, the position reference for the closed-loop system has a trapezoidal shape.
%The closed-loop system performance  depends on the controller gains, and hence, $\vcx$ should be designed such the performance is optimized. 
% The vibration during grinding and the amount of overshoot at arriving or leaving the operation point should be minimized, while the closed-loop system safety is guaranteed. Our aim is to tune the controller gains, $\mathrm{x}$, to achieve this objective (see Section \ref{sec:PF}).
Our aim is to tune the controller gains, $\mathrm{x}$, such that the vibration during grinding and the amount of overshoot at arriving or leaving the operation point should be minimized, while the closed-loop system safety is guaranteed (see Section \ref{sec:PF}).
To this end, based on the closed-loop behaviour of the system, we consider performance metrics illustrated in Figure \ref{fig:cost}.
More precisely, let $\Ts$ denote the sampling time and $e_{\vcx}:[\uk\Ts,\ok\Ts]\to\Rbb$ be the error signal during a cycle of standard operation of the system where the controller gains are set to $\vcx$.
Also, let $\tSP:=\kSP\Ts$ and $\tST:=\kST\Ts$ be  respectively the time instants of arriving or departing the operation location.  
% We do this by treating tuning as an optimisation problem. 
%The decision variable, denoted by $\mathrm{x}$, is the vector of controller gains. 
%
%In other words, $\vcx^*$ should be designed such that the vibration during the grinding as well as the amount of overshoot at arriving or leaving the operation point are minimized, and meanwhile, the safety of the closed-loop system is guaranteed especially during the tuning procedure.
Accordingly, the performance metrics are defined as following 
\begin{itemize}
    \item $\CSP(\vcx)$, the maximum error after departing the operation location, i.e., $\CSP(\vcx) := \max_{\kST+1 \le k}\ |e_{\vcx}(k\Ts)|$,
     \item $\CST(\vcx)$, the overshoot after arriving at operation location,
     i.e., $\CST(\vcx) := \max_{\kSP \le k \le \kST}\ |e_{\vcx}(k\Ts)|$,
     \item$\CSS(\vcx)$, the $L_1$-norm of the position error at the operation location scaled with the sampling time $\Ts$,
     i.e., $\CSS(\vcx) := \Ts \sum_{\kSP \le k \le \kST}\ |e_{\vcx}(k\Ts)|$,
     \item{$C_\text{crit}(\vcx)$, a metric introduced for further enhancing experimental safety (see equation \eqref{eqn:Ccrit}). 
   %  More details are provided in Sections \ref{sec_experiments_1}.
     }
\end{itemize}
\begin{figure}[b]
%\vspace{-3mm}
\centering
\includegraphics[width=0.4\textwidth]{img/Fig4_costfunction1P1_old_v3.pdf}
\caption{Illustration of the three performance metrics on the position error signal (input signal to $C_{\mathrm{p}}(s)$)}
\label{fig:cost}
\end{figure}
Due to static friction,  $\CSP(\vcx)$ has a larger magnitude compared to $\CST(\vcx)$  (see Figure \ref{fig:cost}), however, 
$\CST(\vcx)$ is more sensitive to the instabilities of the system.
Therefore, we additionally consider a constraint $\CST(\vcx) \leq c_{\text{b}}$ for enforcing the safety, where $c_{\text{b}}$ is a pre-decided bound for the maximum allowed overshoot.
Accordingly, we have
\begin{equation}
\vc{c}(\vcx):=[\CSP(\vcx), \CSS(\vcx),\CST(\vcx),\Ccrit(\vcx)]^\tr,
\end{equation}
and the overall performance metric $f(\vcx)$ is defined as the weighted sum introduced in \eqref{eqn:overall_perf}.
From Section \ref{sec:PF}, the optimal controller gains $\vcx^*$ are obtained by solving the following optimization problem
\begin{equation}\label{eqn:CBO_NumVer}
\begin{array}{cl}    
\minOp_{x \in \Xbb}
&
\!\!
f(\vcx):= 
w_1 \CSP(\vcx) \!+\! w_2 \CSS(\vcx) \!+\!  w_3 \CST(\vcx) \!+\!  w_4 \Ccrit(\vcx) 
\\\text{s.t.}
&
\!\!
g(\vcx):=\CST(\mathrm{x}) \leq c_{\text{b}}.
\end{array}
\end{equation}
One can see that functions $f$ and $g$ are in black-box oracle form with respect to $\vc{x}$, i.e., their analytical closed form is not available and one can access their values for a given $\vc{x}$ only by performing an experiment on the machine and a subsequent calculation.
Accordingly, for tuning the controller gains, we utilize the data-driven procedure introduced in Section \ref{sec:BO}. For the numerical experiments, it was sufficient to maintain safety only through the constraint $g(\vcx)$, therefore the weight $w_4$ corresponding to $\Ccrit$ was different than zero only for the experiments on machine.
%Since term $\Ccrit$ is used in the experimental phase, the corresponding weight $w_4$ is set to zero in the numerical experiments. 


%Before providing the details of CBO implementation, we need to highlight the  role of $C_\text{crit}(\mathbf{x})$ which is introduced for experimental safety enhancement by penalizing samples with high proportional gains in the velocity and position controllers. 
The function $C_\text{crit}(\mathbf{x})$ is defined as
\begin{equation}\label{eqn:Ccrit}
C_\text{crit}(\vcx) = \rho_\text{crit}\ \! \exp(\frac{\Kp}{\Kp^\text{crit}})\ \! \exp(\frac{\Kv}{\Kv^\text{crit}}) \, ,
\end{equation}
where $\rho_\text{crit}$ is a scaling factor to adjust the magnitude of the penalty according to the other terms of the cost,  $\Kp^\text{crit}$ and $\Kv^\text{crit}$ are the controller critical gains estimated experimentally during training data collection. $C_\text{crit}(\vcx)$ is a penalization term introduced to incorporate additional information on safety. %\cmr{[move this metric to the experimental part]}

%=============================================
%=============================================
%=============================================
%=============================================
%=============================================
%\vspace{-3mm}
\subsection{Numerical Results}
\label{sec_simulation}

%\cmm{System model and controller} \\
%\cmm{Performance features (+safety measurements) for the system} \\


In this section, we numerically evaluate the performance of the proposed tuning method and compare with competing methods in the literature.
%In this section, we evaluate numerically the performance and safety of the proposed algorithm applied on the linear axis system  modelled and identified in Section \ref{sec_model}. 
%We first obtain the global optimum by grid evaluation in Section \ref{sec_simulation_1} which we later use as a benchmark with respect to the optimum obtained by the proposed algorithm. We further compare the result with two methods for optimization of the acquisition function, namely grid search and particle swarm optimization in Section \ref{sec_simulation_2}. 
%The proposed approach is then compared to the result from relay feedback autotuning method in Section \ref{sec_simulation_3}. 
%Finally, in Section \ref{sec_simulation_3}, we compare the computational performance of the proposed algorithm to another Bayesian optimization algorithm ensuring safe candidate configurations. 
%where we investigate the maximization of the $\alpha_{\text{CEI}}$ acquisition function comparing grid search and particle swarm optimization (PSO) in Section \ref{sec_simulation_2}. Next, we compare the controller performance achieved by BO-tuning using PSO to that achieved by a standard tuning method in \ref{sec_simulation_4}. Finally, we compare the computational performance of constrained BO tuning to another BO algorithm ensuring safe candidate configurations in \ref{sec_simulation_3}.
\subsubsection{Global Optimum and Bayesian Optimization Range}
\label{sec_simulation_1}
First, we use the linear axis model from Section \ref{sec_model} to compute the optimization ranges where the system is stable, and to find the global optimum using grid search. The ranges are later used in the experimental implementation.

In Figure \ref{fig:GX_sim_grid_7p5ms}, the individual cost terms and their weighted sum $f(\vcx)$ are calculated and displayed on a two-dimensional grid $\Kp \times \Kv$ with 320 $\times$ 300 points and resolution $(\Delta \Kp,\Delta \Kv) = (0.25, 0.05)$, for fixed $\Ti = 7.5$ms. %, as for all 2D optimization experiments. 
The computed global optimum is shown on the upper left cost panel. 
\begin{figure}[h]
\centering
\includegraphics[width=0.485\textwidth]{img/Fig5_GX_sim_grid_7p5ms_contourP_new2.pdf}
\caption{2D grid of the individual and combined cost terms using the identified system model, $\Ti = 7.5$ms. The optimum resulting from grid evaluation is shown in the top left panel.}
\label{fig:GX_sim_grid_7p5ms}
%\vspace{-2mm}
\end{figure}
Table \ref{tab:opt_range} shows the parameter values corresponding to the computed optima for $\Kp$ and $\Kv$, while keeping $\Ti$ fixed, and those corresponding to joint exhaustive evaluation on the grid of the three parameters where $\Ti$ is a variable as well. 
The latter finds a solution with lower cost, while the values of the parameters are increased.
 %and the three-dimensional ($\Kp$, $\Kv$, $\Ti$) numerical models, found by particle swarm optimization (PSO).
The range of the parameters' values chosen here 
(see Table \ref{tab:opt_range})
includes the nominal and optimal parameters as well as the stability limits resulting from grid evaluation, where the overshoot criterion is violated.
\begin{table} [h]
 \caption{Global optima and optimization range for the numerical exhaustive evaluation experiments}
 \label{tab:opt_range}
    \centering
    \ra{1.3}
    \begin{tabular}{ @{}l c c c c c c@{} }\toprule
    & 2D optimum && 3D optimum && Range\\
    \midrule
     $\Kp$ [$\mathrm{\frac{1000}{min}}$] & $45.5$ && $57$  &&  $10$ -- $70$\\
     $\Kv$ [$\mathrm{\frac{N}{mm/min}}$] & $5.9$ && $6.85$ && $0.5$ -- $8$\\
     $\Ti$ [ms] & $7.5$ (fixed) && $12.5$ && $5$ -- $17$\\
     Cost $f$ & $1.5048$e-$4$ && $1.3923$e-$4$ && --\\
   \bottomrule
    \end{tabular}
    %\vspace{-2mm}
\end{table}

\iffalse
\subsection{Optimization of the Acquisition Function}
\label{sec_simulation_2}
The main part of the proposed approach is the sampling step performed by finding the optimum of the acquisition function in \eqref{eqn:x_next}. 
This can be done by various methods including nonlinear programming techniques such as limited-memory BFGS \cite{Frazier}, \cite{Liu},  grid search \cite{Gardner}, and global optimization methods like particle swarm optimization \cite{Khosravi}. 
The main drawback of nonlinear programming is being prone to entrapment in local minima when the optimization problem is non-convex, like in  \eqref{eqn:x_next}. 
While the grid search methods have the potential of finding the global optima, the grid evaluation depends strongly on the resolution and the dimension of the grid. 
%The optimum of the acquisition function \eqref{eqn:x_next} can be found by various methods, e.g., limited-memory BFGS \cite{Frazier}, \cite{Liu},  grid evaluation \cite{Gardner}, or  particle swarm optimization \cite{Khosravi}. 
%The limited-memory BFGS methods are designed to minimize smooth functions without constraints, and grid evaluation depends strongly on the resolution and the dimension of the grid. 
Finally, the particle swarm optimization (PSO) is a global optimization method that can be adapted to constraints, works in continuous space, and scales well with the dimensionality of the problem \cite{Kennedy}.
Table \ref{tab:PSO_comp} shows a comparison of the PSO method using 10 particles with a grid-based evaluation for different resolutions of the grid in the numerical CBO experiments following the cost without safety penalization for 10 repetitions. 
Each trial starts with the same initial set of 25 points, drawn by Latin hypercube sampling. 
For all experiments the parameters $\Kp$, $\Kv$ and $\Ti$ are optimized simultaneously. 
For grid maximization, the values are discretized according to the resolution of the grid. 
When a fine resolution is used, the PSO algorithm is computationally faster and terminates closer to the optimum with a higher number of iterations. 
Note that the number of iterations is balanced with the final cost value through the termination criterion \eqref{eq:stop_aCEI}. 
Solving  \eqref{eqn:x_next} using a coarse grid optimization achieves smaller number of iterations and less computational time comparing to PSO, again with higher cost compared to the PSO result. 
It is empirically observed that improving the resolution of the grid by factor two in all three dimensions increases the computational time by factor 6, while the PSO is not limited to a grid resolution.
On other hand, regarding the performance of PSO with larger swarm population, similar results are obtained when 100 particles are used.

\begin{table} [h]
\caption{Comparison of PSO and grid search for acquisition function optimization (mean and 95\% confidence interval)}
\label{tab:PSO_comp}
    \centering
    \ra{1.3}
    \begin{tabular}{ @{}c c c c c @{} }\toprule
        & median & median & \\
     search method & num. of iter. $N$ & comp. time~$t$ [s] & cost $f$\\
     \midrule
     grid search & & &\\
     240$\times$75$\times$4 & $39$ & $45.2$ & $1.47\text{e-}4\pm1.01\text{e-}5$\\\midrule
     grid search & & &\\
     480$\times$150$\times$8 & $32$ & $172.5$ & $1.46\text{e-}4\pm 1.1\text{e-}5$\\\midrule
     PSO 10 particles & $49.5$ & $115.84$ & $1.45\text{e-}7\pm 9.63\text{e-}6$\\
   \bottomrule
    \end{tabular}
\end{table}
  % When a limit of iterations ($N_\text{limit}$ = 50) is used instead of the termination criterion, the PSO and grid search algorithm with coarse resolution ($\Delta \Kp$ = 0.25, $\Delta \Kv$ = 0.1) perform equally in terms of computational time and optimality error. 
%(see Figure \ref{fig:GX_sim_grid_pso_comp2}). Since the grid search algorithm is faster in this two-dimensional problem, it would be the better choice in this case, otherwise the number of particles can also be reduced for the PSO. In this work we use PSO as maximization method of the acquisition function. Whenever run time is of high importance, grid evaluation can be used also in a low dimensional problem.

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.25\textwidth]{img/GridPSO_comp1new.pdf}
%\caption{Comparison of grid search and %PSO to maximize the acquisition function %with fixed number of iterations %$N_{limit}$ = 50}
%\label{fig:GX_sim_grid_pso_comp2}
%\end{figure}
% To do
Figure \ref{fig:GX_sim_grid_pso_comp} shows that the optimized gains are spread in the vicinity of the the optimal controller parameters.
This typical feature of the proposed tuning is due to the flat shape of the graph of the cost function over this region.
The stopping criterion can be modified to tighten the final allowed optima while balancing the number of the required iterations for reaching to the optimal gains.
\begin{figure}[h]
\centering
  \includegraphics[width=0.75\linewidth]{img/Fig6_GridPSO_comp_contourP_new1.pdf}
\caption{Comparison of grid search and PSO to maximize the acquisition function}
\label{fig:GX_sim_grid_pso_comp}
\end{figure}
\fi
\subsubsection{Comparison with Relay Feedback Tuning}
\label{sec_simulation_4}
For the next numerical experiment we compare the proposed method with relay feedback tuning which is a benchmark controller (auto)tuning approach 
%for cascade control 
\cite{Hang3}. The relay feedback tuning is fully deterministic, robust to the disturbances, and tunes simultaneously the three parameters of the position and velocity controller $\Kp$, $\Kv$ and $\Ti$. 
The tuning procedure depends on information automatically extracted from the frequency response of the plant, which is generally sufficient for PID controller tuning of many processes \cite{Hang2,Hang3}. 
One may utilize the relay method for nonlinear processes when it is possible to tune the relay parameters to keep the system in a region with approximately linear behavior.
%With an appropriate choice of relay parameters, relay feedback autotuning can be held close to the set-point of the system in an approximately linear region, which makes the method suitable for control of nonlinear processes \cite{Astrom}. 

%Here we use it as a comparison benchmark for the performance of the proposed tuning method. 
%Moreover it has been shown that the relay feedback auto-tuning can be modified to cope with disturbances and perturbations \cite{Hang2},\cite{Shen},\cite{Park}. 
Table \ref{tab:RF_comp} shows the results of ten simulated experiments with different training samples drawn using Latin hypercube sampling for the joint optimization of $\Kp$, $\Kv$ and $\Ti$ in comparison with relay feedback tuning. We use particle swarm optimization to optimize the acquisition function.
\begin{table} [t]
\caption{Comparison of the parameters, cost and number of iterations between the proposed method with $\vc{w}=\frac{1}{4}(1,1,2,0)^\tr$ and relay feedback tuning (mean and 95\% confidence interval% are shown.
)}
\label{tab:RF_comp}
    \centering
    \ra{1.3}
    \begin{tabular}{ @{}l c c c c@{} }\toprule
   Parameter & CBO && Relay feedback\\ \midrule
     $\Kp$ [$\mathrm{\frac{1000}{min}}$] & $57.64\pm5.67$ && $41.72$\\
     $\Kv$ [$\mathrm{\frac{N}{mm/min}}$] & $6.48\pm 0.77$ && $3.64$\\
     $\Ti$ [ms] & $13.90\pm 0.32$ && $16.80$\\
     Cost $f$ & $1.48$e-$4 \pm 0.11$e-$4$ && $2.78$e-$4$\\
     Number of iterations $N$ & $71 \pm 31$ && $1$\\
   \bottomrule
   %\vspace{-2mm}
    \end{tabular}
    %\vspace{-4mm}
\end{table}
Since the proposed tuning method is performance-based, the cost is 48\% lower than the corresponding cost of the parameters tuned by the relay feedback procedure. 
However, the algorithm requires between 40 and 100 iterations in addition to the 25 evaluations of the initial set, while the relay feedback method calculates the parameters from a single response of the system \cite{Khosravi2020,Khosravi2020b}. 
Accordingly, one can leverage the benefit of the proposed method especially when the machine performs a repetitive task.
Both methods can be fully automated, and could be selected depending on the performance of the system and the duration of the tuning procedure.

% Excluded
%\begin{comment}
% BO convergence and motivation behind the relative termination criterion (cut or put in sec_03_bo?)
%Figure \ref{fig:GX_sim_meancon} illustrates the convergence of the maximum of the CEI acquisition function and the variance of the cost at each candidate during all BO iterations in four different calculations. Since the CEI levels are different for each BO experiment, it is difficult to determine an absolute threshold of the CEI maximum as termination criterion. Furthermore, the CEI level can increase during the BO, when the prediction does not match the real value of the cost. Thus, the relative threshold on the CEI maximum w.r.t. the CEI maximum over all iterations is chosen for this work (see \eqref{eq:Stop}). To cope with the sudden increases of the CEI maximum after dissonance between prediction and real cost, the relative threshold has to be matched in three consecutive iterations.

%\begin{figure}[H]
%\centering
%\includegraphics[width=0.8\textwidth]{img/GX_sim_meancon.pdf}
%\caption{BO prediction, real cost values and maximum CEI over all iterations during four BOs on the GX simulation model}
%\label{fig:GX_sim_meancon}
%\end{figure}

%To further improve the GP prediction the hyperparameters can be retuned at every iteration, this however disturbs the convergence of the CEI maximum and therefore the termination of the BO algorithm. Thus, the hyperparameters are tuned only once after the training data sampling.
%\end{comment}

%\vspace{-0mm}
\subsubsection{Safety and Stability}
\label{sec_simulation_3}
Avoiding unstable parameter values, and keeping the system safe is critical both during tuning and operation. 
We explored tuning using an adaptation of SafeOpt, a BO-based algorithm for safe exploration of the parameter space \cite{Duivenvoorden}. The SafeOpt algorithm starts with an initial safe set and uses two different acquisition functions for sampling. The first one is defined based on the lower confidence bounds obtained from Gaussian process model of the objective function, and it is designed to find candidate optimizers. 
The second acquisition function is for exploring the domain and expanding the safe set of the parameters. This acquisition function is defined based on the confidence bounds obtained for the safety constraint, and penalizes candidate points which are probably unsafe. Hence, the input parameters fulfilling the safety constraints are selected with high certainty. 
\begin{figure}[h]
\centering
\includegraphics[width=0.42\textwidth]{img/Fig10a.pdf}
\caption{Comparison of the convergence of the CBO algorithm with SafeOpt}
\label{fig:GX_sim_SafeOpt_comp}
\end{figure}
Figure \ref{fig:GX_sim_SafeOpt_comp} shows the performance achieved by SafeOpt and by constrained Bayesian optimization using $f(\vcx)$ for the optimization of $\Kv$ and $\Kp$. 
A training set of 15 measurements is selected by Latin hypercube sampling inside the range $20 \leq \Kp \leq 52.5$ and $1 \leq \Kv \leq 6$, computed using grid evaluation, to avoid areas that violate the constraint. 
The SafeOpt particle swarm implementation uses the samples of the initial set as safe starters. 
The hyperparameters of both algorithms are tuned by minimization of the negative log marginal likelihood, after evaluation of the initial set. 
In a second series of refined SafeOpt experiments, the hyperparameters of the constraint are fixed to more conservative values, namely smaller length-scales and higher signal variance, resulting in higher uncertainty outside known regions.

Each optimization experiment terminates after running a fixed number of 50 iterations. At the end of the 50 iterations both implementations of the SafeOpt algorithm, including experiments that start with better values inside the training set, remain with higher cost as compared to CBO.
SafeOpt needs to complete PSO three times for every iteration (see \cite{Duivenvoorden} for more details), which increases the computational time. 
Due to the large distance between the optimum and the constraint, SafeOpt with tuned hyperparameters results in more constraint violations than the CBO algorithm (see Table \ref{tab:SafeOpt_comp}), because SafeOpt actively tries to expand the safe optimization range of the function and thus also chooses samples near the boundary of feasible set. 
The constraint violations can be reduced 
%to zero 
by fixing the hyperparameters, which leads to slower convergence. 
We have thus adopted CBO in combination with additional safety measures for the real system.
% \begin{comment}
% \begin{table} [h]
% \caption{Comparison of CBO with SafeOpt (mean and 95\% confidence interval)}
% \label{tab:SafeOpt_comp}
%     \centering
%     \ra{1.3}
%     \begin{tabular}{ @{}l c c c c@{} }\toprule
%     & CBO & SafeOpt & SafeOpt\\
%     & & (tuned) & (conservative)\\\midrule
%      Final cost & 1.504e-4 $\pm$ 5.586e-7 & 1.55e-4 $\pm$ 2.076e-6 & 1.593e-4 $\pm$ 1.282e-5\\
%      Computational time (median) [s] & 303.5 & 710.2 & 707.3\\
%      Constraint violations (median) & 1 & 5 & 0\\
%   \bottomrule
%     \end{tabular}
% \end{table}
% \end{comment}
\begin{table} [t]
\caption{Comparison of CBO with SafeOpt for the optimization of $\Kp$ and $\Kv$ (mean and 95\% confidence interval).}
\label{tab:SafeOpt_comp}
    \centering
    \ra{1.3}
    \begin{tabular}{ @{}l c c c c@{} }\toprule
     & & Median & Median\\    
     & Final cost & comp. time & constr. violations\\ \midrule
    % & & time [s] & violations\\\midrule
     CBO & 1.50e-4 $\pm$ 5.59e-7 & 303.5 & 1\\
     SafeOpt (tuned) & 1.55e-4 $\pm$ 2.08e-6 & 710.2 & 5\\
     SafeOpt (fixed) & 1.59e-4 $\pm$ 1.28e-5 & 707.3 & 0\\
   \bottomrule
   %\vspace{-4mm}
    \end{tabular}
    %\vspace{-2mm}
\end{table}

==> New version Safety-aware BO - arXiv/sections/sec_05_results_exp.tex <==

%\vspace{-4mm}
\section{Experimental Results}
\label{sec_experiments}

\iffalse
\begin{figure}[h]
\centering
\includegraphics[width=0.25\textwidth]{Figs/Dom_Setup.pdf}
%\caption{Iteration over $\Kp$, fix $\Kv$ = 1 ($\Kp^\text{crit}$ = 38)}
%\caption{Iteration over $\Kv$, fix $\Kp$ = 20 ($\Kv^\text{crit}$ = 1.8)}
\caption{Grinding machine used in the experiments.}
\label{fig:GX_detcrit}
\end{figure}
\fi 






%Add here
%%The nominal controller settings used in the model and in the real system for the position P and velocity PI controller are ($K_\text{p}^\text{nom}$ = 20$\mathrm{\frac{1000}{min}}$, $K_\text{v}^\text{nom}$ = 1$\mathrm{\frac{N}{mm/min}}$, $T_\text{i}^\text{nom}$ = 7.5ms).

We now demonstrate the tuning method on the linear axis drive. First, we introduce the system where we do experimental validation. We then present the adaptation needed to safely operate and reach stable parameters. Finally, we examine the convergence of the algorithm.

%\vspace{-2mm}
\subsection{Experimental System}
\label{sec:exper_system}
Our experimental system is a linear axis drive integrated in a DomSemi grinding machine (see Figure \ref{fig:machine_axes}) for face grinding from Agathon AG, steered by a controlled brushless permanent magnet AC motor.
The position and velocity measurements are provided with an optical sensor system with precision of $100$nm.
% An optical encoder measurement system with resolution of 100 nm provides the position and velocity measurements. 
The nominal controller settings used in the model and in the real system for the position P and velocity PI controller are ($\Kp^\text{nom}=20~[\mathrm{1000/min}]$, $\Kv^\text{nom}1~[\mathrm{N /(mm/min)}]$, $\Ti^\text{nom} = 7.5~[\text{ms}]$).
%
The position, velocity and force of the linear axis drive are limited by the controller to a $137$mm range, $315$mm/s speed and $400$\% of the motor power in both directions, respectively. 

\subsection{Critical Gain Detection}
\label{sec_experiments_1}

We implement the tuning method using the optimization as formulated in \ref{eqn:CBO} to tune $\Kp$ and $\Kv$. The corresponding weights in the cost are $\vc{w}:=\frac{1}{4}(1,1,2,0)^\tr$. We restrict the tuning on the real system in the range $20 \leq \Kp \leq 52.5$ and $1 \leq \Kv \leq 6$, computed using our numerical model with grid evaluation. The left panel of Figure \ref{fig:GX_prediction_exp} shows the resulting GP model of the cost after completing all tuning iterations, along with the corresponding optimized controller parameters. The optimum $(\Kp,\Kv) = (27.75,1.43)$ is located right at the limit of the safe range, as can be seen on the left panel of Figure \ref{fig:GX_prediction_exp}. While this is acceptable in the tuning mode, during actual grinding the performance can shift due to additional loads and forces, and the optimum could accordingly become unsafe. Routinely this is overcome by selecting conservative controller parameters, which in turn curbs the system's performance.
%The optimum, corresponding to $(\Kp,\Kv) = (27.75,1.43)$, found by the proposed tuning approach, using $f(\vcx)$ with $\vc{w}:=\frac{1}{4}[1,1,2,0]^\tr$, is located right at the limit of the safe range, as can be seen on the top panel of Figure \ref{fig:GX_prediction_exp}.
\begin{figure}[t]
\centering
\includegraphics[width=0.485\textwidth]{img/Fig8_GX_prediction_critw0_contour1P_2.pdf}
\caption{Predicted cost for tuning on the actual axis with and without penalty. The optima are shown by black circles.}
\label{fig:GX_prediction_exp}
%\vspace{-5mm}
\end{figure}

We incorporate this additional uncertainty by increasing the weight for the safety penalty $C_{\mathrm{crit}}$ from $0$ to $1/3$ and by adapting the remaining weights. We determine the critical gains in the $C_{\mathrm{crit}}$ by monitoring the fast Fourier transform (FFT) of the position error in a fixed frequency window. This comprises an initial scan for all gain parameters, starting from the nominal values and increasing until a threshold of $0.4$mm in the FFT of the position error is exceeded, as shown in Figure \ref{fig:GX_detcrit}. The critical gains in each loop are determined in consecutive scans, while keeping the parameters of the inner loop fixed, therefore discarding the mutual dependence of the controller's parameters. 
\begin{figure}[h]
\centering
\includegraphics[width=0.485\textwidth]{img/Fig9_GX_detcrit_Kp_KvP.pdf}
%\caption{Iteration over $\Kp$, fix $\Kv$ = 1 ($\Kp^\text{crit}$ = 38)}
%\caption{Iteration over $\Kv$, fix $\Kp$ = 20 ($\Kv^\text{crit}$ = 1.8)}
\caption{FFT of the position error signal for different controller gains, with the corresponding threshold indicated with a dashed line. The bottom panels are examples of reaching the critical gain, following consecutive scanning for $\Kv$ and $\Kp$.}
\label{fig:GX_detcrit}
\end{figure}
Once these gains are known, the cost penalization in \eqref{eqn:CBO} is applied. The right panel of Figure \ref{fig:GX_prediction_exp} shows the %corresponding 
GP model predictions of the cost $f(\vcx)$ with %corresponding weights of
weights
$\vc{w}:=\frac{1}{6}(1,1,2,2)^\tr$, after collecting the data from all BO iterations on the real system, along with the optimized controller gains. 
In this case, the optimization range  is limited and depends on the detected critical gains in the scanning phase, i.e., $\Kp\le 0.75 \ \! \Kp^\text{crit}$ and $\Kv\le 0.75 \ \! \Kv^\text{crit}$. This is the range used for both panels in Figure \ref{fig:GX_prediction_exp}.
\subsection{Convergence of Method}
\label{sec_experiments_2}
\begin{figure}[h]
\centering
\includegraphics[width=0.4\textwidth]{img/Fig10_GX_experimentBO_meanconPb.pdf}
\caption{The predicted cost, real cost and maximum CEI over all iterations of the proposed tuning algorithm on the real grinding system.}
\label{fig:GX_experimentBO_meancon}
%\vspace{-4mm}
\end{figure}
The convergence of the constrained expected improvement (CEI) maximum and the variance of the CEI maximum candidate cost (the predicted mean of the cost) are illustrated in Figure \ref{fig:GX_experimentBO_meancon} for each iteration of the proposed tuning scheme, and the acquisition function evolution is included as well. 
The predicted mean of the cost decreases with the number of iterations, and already at the fourth iteration is virtually identical to the experimentally determined cost. 
After the CEI maximum of the current iteration drops under 5\% of its maximal value in iteration 3, which is the threshold set in the stopping criterion \eqref{eq:stop_aCEI}, and stays there for 3 consecutive iterations, the algorithm is terminated after iteration 5. Although the minimum of the cost happens at iteration 3, the stopping criterion which depends on the CEI changes between iterations is only fulfilled at iteration 5.
Therefore, the algorithm needs five iterations to fulfill the stopping criterion, 26 experiments for finding the critical gains and the initial set of 15 experiments for training of the GP model of the cost, resulting in 46 experiments in total. The resulting performance is significantly improved, as shown in Figure \ref{fig:cost}. All performance metrics are improved, especially the initial overshoot $C_{ST}$ shows a decrease of 50 \%. The frequency domain plot shows that the found parameters are stable without introducing vibrations (e.g. high-frequency components remain low), and exemplifies the decrease in the low-frequency range, corresponding to improved tracking.

Upon re-tuning only a small number of experiments will be needed to account for changes in the system. The old experiments can still be used as prior information.

\begin{figure}[ht]
\centering
\includegraphics[width=0.45\textwidth]{img/before-after1.pdf}
\caption{The position error signal and the improvement of each metric before and after tuning, in time-domain (left), and the position error signal in frequency domain (right).}
\label{fig:cost}
%\vspace{-4mm}
\end{figure}
\iffalse
\begin{table} [t]
\caption{Comparison of the metrics, before and after tuning}
\label{tab:metric_comp}
    \centering
    \ra{1.3}
    \begin{tabular}{ @{}l c c c c@{} }\toprule
        & nominal & tuned &  [\%]\\ \midrule
     $C_{SP}$ & 5.6e-3 & 4.2e-3 & $	\downarrow$25\\
     $C_{SS}$ & 7.4e-5 & 4.7e-5 & $	\downarrow$36.5\\
     $C_{ST}$ & 4e-4 & 2e-4 & $	\downarrow$50\\
   \bottomrule
    \end{tabular}
\end{table}
\fi
\iffalse %\iftrue
\subsection{Performance evaluation in grinding}
\label{sec_experiments_3}
The tuning procedure is carried out in a specific operating mode in which the loads and forces differ from those in grinding mode. We now study the grinding performance of the machine, both for nominal/conservative gains, and for the CBO-tuned gains (see table \ref{tab:GX_Grind_rad}). A polycrystalline cubic boron nitride (PCBN) workpiece is used to test the grinding of a rectangular workpiece with rounded corners, where each corner has a different radius, as shown in Figure \ref{fig:GX_Grinding_rad}. %PCBN has a hardness of 4000HV at room temperature \cite{Abrao}. 
%\caption{Position error and force measurement of the encoder}
%\label{fig:GX_Grinding_rad_1}
%\caption{Surface error measurement of Confovis 3D microscope for 1.6mm radius}
%\label{fig:GX_Grinding_rad_2}

The position error measured by the encoder data shown in the top panel of Figure \ref{fig:GX_Grinding_rad} is a suitable first indicator of grinding performance. This position error is higher for the nominal parameters, as compared to the same error  achieved with BO-tuning, critical gain detection and safety term in the cost. The BO-based tuning parameters without the safety term achieve even lower position error while maintaining comparable grinding force throughout the trial, which can be explained by the more agressive control parameters that only consider performance criteria. Because the encoder measurement is more indirect of the final quality, as it takes place away from the grinding process, and accounts mostly from mechanical effects in the system, but not for the grinding process influence,  we chose the surface error measurement of the ground workpiece from a 3D microscope, which is a standart quality control metric. The inspection of the 1.6mm radius with the Confovis 3D microscope shows a higher surface error for the BO parameters without the safety term, than for the nominal parameters, whereas the BO parameters with the safety term result in less or similar surface error as the nominal parameters (see Figure \ref{fig:GX_Grinding_rad} and table \ref{tab:GX_Grind_rad}). 
\begin{table}[h] % Change for twocolumn design
 \caption{Gains of the different parameter configurations and surface error of the 1.6mm radius measured by the Confovis 3D microscope measurement}
 \label{tab:GX_Grind_rad}
    \centering
    \ra{1.3}
    \begin{tabular}{ @{}l c c c c c @{} }\toprule
  %& $\Kp$ [$\mathrm{\frac{1000}{min}}$] & $\Kv$ [$\mathrm{\frac{N}{mm/min}}$]\\
 & Nominal gains  & $K^\text{crit}_1$  &  $K^\text{crit}_2$ & $K_{BO_{sim}}$\\ \midrule
$\Kp$ $[\frac{1000}{min}]$ & 20 & 18.25 & 22.03 & 27.75 \\
$\Kv$ $[\frac{N}{mm/min}]$ & 1 & 1.24 & 1.09 & 1.425 \\
Max absolute error $[\mu m]$ & 3.50 & 2.90 & 3.20 & 4.31 \\
Mean absolute error $[\mu m$] & 0.95 & 1.13 & 0.90 & 1.42 \\  \bottomrule
    \end{tabular}
\end{table} 
\begin{figure}[H]
\centering
\includegraphics[width=0.37\textwidth]{img/GX_Grinding_rad_all.pdf}
\caption{Performance during grinding of 0.4mm, 0.8mm, 1.6mm and 3.2mm radii}
\label{fig:GX_Grinding_rad}
\end{figure}
%\end{comment}
\fi % of iftrue/iffalse end




==> New version Safety-aware BO - arXiv/sections/sec_06_discussion.tex <==
\iffalse
\section{Discussion}
\label{sec:discussion}
% Based on the proposed method and observed performance, 
Constrained Bayesian optimization has been applied to tune a cascaded controller in a model-free approach, while ensuring  safety  by  experimentally  determining  the  critical gains  of  the  controller and adapting the optimization range to more conservative values. 
Scanning in advance for the determination of the critical gains provides the means to inform the Bayesian optimization about safety and stability bounds in the system. 
With the current method, the coupling between the parameters of the position and velocity controllers is not considered. 
Measuring in addition the force signal without fixing the inner loop parameters could provide an improved approximation of the critical gains, and is a topic of future research. 
The proposed algorithm can run autonomously, between production cycles, without disturbing the operation of the system.
If the system undergoes large physical changes between tuning cycles, the pre-learned critical values might not be accurate. 
If such changes are expected, they can be accommodated in a modified version of the proposed tuning scheme through incorporation of a multi-task BO algorithm \cite{Multi-taskBO} where different task parameters can account for changes once the algorithm is informed, and the prior models can be transferred, instead of re-learning them from scratch. 
Similarly, if there are significant variations between different systems, they can be represented through a task parameter, thus simplifying the learning procedure and reducing the number of samples needed for the model of the GP priors.
\fi

==> New version Safety-aware BO - arXiv/sections/sec_07_conclusion.tex <==
\section{Conclusion}

Constrained Bayesian optimization has been applied to tune a cascaded controller in a model-free approach, while ensuring safety  by  experimentally determining  the  critical gains  of the controller. 
Scanning in advance to determine the critical gains provides the means to inform the Bayesian optimization about safety and stability bounds in the system. The proposed algorithm can run autonomously, between production cycles, without disturbing the operation of the system.
If the system undergoes significant physical changes between tuning cycles, the pre-learned critical values might not be accurate. The proposed algorithm can then be extended to accommodate such changes by incorporating task (context) parameters in the modeled system performance.  This extension enables the transfer of the prior models instead of re-learning them from scratch.  
With the current method, the achieved performance exceeded the nominal one by more than 20\%, while automating and standardizing the tuning procedure.
\vspace{-2mm}

%With the current method, the coupling between the parameters of the position and velocity controllers is not considered. Measuring in addition the force signal without fixing the inner loop parameters could provide an improved approximation of the critical gains, and is a topic of future research. 


%A data-driven auto-tuning method for cascade control, using constrained Bayesian optimization was presented and demonstrated on a linear axis drive. To avoid instabilities upon modifications in the system, a method to detect the critical gains was developed, using the fast Fourier transform (FFT) of the position error measurement. The optimization objective of the CBO algorithm was expanded by a term depending on the calculated critical gains, penalizing gains close to critical and maintaining stability and safety during the optimization.

%Further research will address tuning of additional parameters e.g. filter bandwidth and current controller parameters, and the integration of additional performance metrics to improve further the efficiency of the algorithm.

%Compared to relay feedback tuning, the algorithm finds controller parameters that achieve better performance. It also shows faster convergence towards the global optimal parameters as compared to safe Bayesian optimization (SafeOpt) tuning.

%The algorithm was experimentally validated on a  CNC grinding machine, where it required an adaptation to maintain safety during grinding. 

%The resulting optimized controller parameters of the extended CBO algorithm were used in a grinding experiment to evaluate the achieved performance during production. The achieved grinding surface error was smaller or equal to the grinding surface error corresponding to the nominal parameter configurations, thus enabling the proposed method as a solution to standardize and automate the cascade controller tuning procedure.

%In this thesis a data-driven auto-tuning method, using constrained Bayesian optimization (CBO) for standardization of a cascade control structure is developed and tested in simulation and on-machine experiments. The objective of the algorithm is to find the optimal position and speed controller gains for the grinding axes of a state-of-the-art CNC grinding machine. In order to archive this, models of the axes are created and the algorithm is tested on the simulation. Furthermore, it is compared with other auto-tuning methods and with the global optimal parameters, computed by particle swarm optimization (PSO). The maximization of the constrained expected improvement (EIC) acquisition function is tested with grid search and PSO and compared. The algorithm is further implemented and adapted on the actual CNC grinding machine and its limitations are illustrated. The resulting parameters are used in a grinding experiment and evaluated. %Furthermore, the algorithm is tested to detect faulty conditions on the machine.

%It is found, that the CBO algorithm results in better performance than a relay feedback tuning and converges faster to the global optimum than a safe Bayesian optimization algorithm (SafeOpt). To maximize the EIC acquisition function using PSO results in better performance than using grid search. Thus, the PSO is implemented, although the grid search algorithm shows slightly faster convergence. On the machine, additional loads and forces, resulting from a grinding process are not reflected in the tuning process and can result in a higher surface error during grinding for the optimal parameters of the tuning process, because of their proximity to the critical gains. An algorithm to detect the critical gains has been developed, using the fast Fourier transform (FFT) of the position error measurement. The performance metric of the CBO algorithm has been expanded by a term depending on the calculated critical gains to cope with this problem. The grinding surface error of the expanded CBO algorithm is smaller or equal than the grinding surface error resulting from the nominal parameter configurations, archived by manual tuning and thus the algorithm can be used as a standardized auto tuning method on the machine. %Furthermore, the algorithm can detect faulty conditions, like a decreased stiffness, due to loose screws in the system and a commutation error of the permanent magnetic drive, if these faults result in a detectable change of the critical gains or the position measurement.

%This thesis outlines the advantages and limitations of using Bayesian optimization for the auto-tuning of cascade PID controllers. To further validate the results of this work, the CBO algorithm needs to be employed on different systems. Moreover, it can be extended and applied to different control architectures. It can further be tested with additional parameters of the system. Furthermore, additional constraints or performance metrics (e.g. based on the force signal) can be implemented in the optimization algorithm to safely cope with the loads and forces from grinding, further improving the performance of the algorithm.% and the detection of faulty conditions of the system.


==> New version Safety-aware BO - arXiv/sections/sec_08_acknowledgements.tex <==
\iffalse
\vspace{-20 pt}
\section{Acknowledgement}
We greatfully acknowledge the support of Agathon AG in providing the equipment necessary to validate the approach and in discussions about the performance metrics.
\fi 

